Geometric Sample Reweighting for Monte Carlo Integration

We present a general sample reweighting scheme and its underlying theory for the integration of an unknown function with low dimensionality. Our method produces better results than standard weighting schemes for common sampling strategies, while avoiding bias. Our main insight is to link the weight derivation to the function reconstruction process during integration. The implementation of our solution is simple and results in an improved convergence behavior. We illustrate its benefit by applying our method to multiple Monte Carlo rendering problems.

==> 06-implementation.tex <==
% %%------------------------------------------------------------
% %
% %
% %%------------------------------------------------------------
% %\subsection{Dispersion}
% %\label{sec:result:dispersion}
% %
% %%------------------------------------------------------------
% %\subsection{Depth of Field}
% %\label{sec:result:depthoffield}
% %For aperture samples within the same pixel, we build a $2$D Voronoi based on the primary samples.
% %The integrator is built on top of a regular path tracer.
% %We tested our aperture sampling with geometric sample reweighting with a glossy dragon model.
% %The camera is focusing on the head part of the model, leaving the rest of the model in defocus blur.
% %See Figure \ref{fig:result:dragon} for a visual comparison and the statistics.
% %
% %\begin{figure*}[tbp]
% %	\centering
% %	\mbox{} \hfill
% %	%\includegraphics[width=\textwidth]{img/6_2_dragon}
% %	\includegraphics[width=\textwidth]{img/6_2_dragon_new}
% %	\caption{The Dragon scene. Glossy Dragon crosses the focal plane of the camera. All four images are rendered with $256$ samples per pixel. Pay special attention to the fallout regions, e.g., highlighted regions.}
% %	\label{fig:result:dragon}
% %\end{figure*}
% %
% %Similar to previous section, the most noticeable difference happen in the falloff regions.
% %Sampling according to function gradient w/ geometric reweighting consistently outperforms its counterparts.

% %%------------------------------------------------------------
% %\subsection{Anti-aliasing Effect}
% %\label{sec:restult:antialising}
% %Primary samples that are used to generate pixel samples ($2$D positions within pixel regions) generated within the same pixel are collected and used to build a Voronoi diagram.
% %On top of a regular path tracer, this implementation mainly targets at object boundaries regions that are not perfectly aligned horizontally or vertically with pixels.
% %See Figure \ref{fig:result:antialiasing} for visual results and comparison.
% %
% %\begin{figure*}[tbp]
% %	\centering
% %	\mbox{} \hfill
% %	\includegraphics[width=\textwidth]{img/6_3_anti_aliasing}
% %	\caption{The cropped Cornell scene. All edges in view are tilted, thus prune to alias. Pay attention to, especially the long semi-horizontal edge. See how weighted result gives a smooth gradient that unweighted one.}
% %	\label{fig:result:antialiasing}
% %\end{figure*}
% %
% %Notice in object boundaries regions, re-weighted results converge faster towards reference: at low sample rate of $64$, re-weighted result already gives a smooth gradient whereas unweighted results still struggle to converge.
% %However, we do notice that uniform samples with reweighting outperforms non-uniform samples with reweighting.

% %%------------------------------------------------------------
% %\subsection{Direct Illumination}
% %\label{sec:restult:lightSampling}

% %-------------------------------------------------------------------------
% \subsection{Discussion}
% \label{sec:implementation:discussion}
% In all above experiments, we observe better performance by reweighting uniform samples.
% Our geometric sample reweighting technique effectively and sufficiently reduces variance and is unbiased.

% However, we do observe the recurring pattern that uniform samples for reweighting are in general more robust and promising than non-uniform samples, be it value driven or gradient driven.
% This agrees with the common sense that some times the uniformity is the key to the solution.
% However, we do not take low discrepancy sample sequences and quasi random samples into comparison, since they are generally considered as being biased.

% We also observe that gradient driven distributed samples almost always outperform samples following value driven distribution.
% This not only agrees with our intuition that more samples should be placed where variation of function is more severe, but also challenges the widely adopted philosophy of value driven importance sampling.

% % ============================================================================
% % End of 06-implementation.tex 
